Dynamic Center-of-Mass Displacement in Aerial Manipulation: An Innovative Platform Design

Aerial manipulators are increasingly used in contact-based industrial applications, where tasks like drilling and pushing require platforms to exert significant forces in multiple directions. To enhance force generation capabilities, various approaches, such as thrust vectoring and perching, have been explored. In this article, we introduce a novel approach by investigating the impact of varied CoM (Center of Mass) locations on an aerial manipulation system's force exertion. Our proposed platform features a design with a dynamically displacing CoM, enabling a smooth transition between free flight and high-force interactions supported by tilting back rotors. We provide detailed modeling and control strategies for this design and validate its feasibility through a series of physical experiments. In a pushing task, the proposed system, weighing 3.12kg, was able to stably exert over 28N of force on a work surface-nearly equivalent to its gravitational force-achieved solely through the tilting of its back rotors. Additionally, we introduce a new factor to evaluate the force generation capabilities of aerial platforms, allowing for a quantitative comparison with state-of-the-art systems, which demonstrates the advantages of our proposed approach.

==> texts/05_simulation.tex <==
% \section{\new{Numerical Results}}\label{sec:validation}
% \new{In this section, simulations that closely emulate the physical platform displayed in \new{Fig.}~\ref{fig:physical_model} are performed to validate the proposed system and control design before moving to real-world experiments. Moreover, risky scenarios including the \ac{com} self-displacing process and complex tool manipulation tasks are tested in simulations to avoid platform damage.} \new{We use} a Simscape model, as in \new{Fig.}~\ref{fig:action}, \new{while the} controller design\new{ed} in \new{Sec.}~\ref{sec:control} and the self-\new{displacing} approach in \new{Sec.}~\ref{sec:com_locate} are implemented in Simulink \new{ running at 100 Hz}. \new{A 2-\ac{dof} manipulation arm equipped with a heavy tool at the \ac{ee} is mounted on the shifting-mass plate, potentially serving for a drilling task. The total system mass and the shifting mass used in the simulation are the same as the physical platform, where $m=3.12$\si{\kilogram} and $m_S=0.9$\si{\kilogram}. The simplified schematic of the manipulator is shown in Fig.~\ref{fig:joints}. We define $L_1$, $L_2 \in \mathbb{R}^+$ as the length of two beams, and $\tau_1$, $\tau_2 \in \mathbb{R}^+$ as the magnitude of joint torques.} The tests include both free-flight evaluations and two physical interaction tasks.

% \new{As the tracking errors from free flights are later displayed from the physical experiments, we now focus on the physical interaction tasks. In \textbf{task 1}, the platform pushes on a vertical work surface using the alignment frame, and the \ac{com} self-displacing approach is conducted to find the ideal shifting-mass plate position for the current setup. In \textbf{task 2}, the manipulator is used to push on the vertical work surface before and after the \ac{com} displacement for benchmarking.}
% \begin{figure}[b]
%    \centering
% \includegraphics[trim={0.15cm 0.1cm 1.9cm 0.4cm},clip,width=\columnwidth]{imagines/plots/interaction_mod.pdf}
%     \caption{\new{\textbf{Task 1}:} the tilting angle $\alpha$ \new{(on the left)} and shifting-mass \new{plate} position $l$ \new{(on the right) evolution during the interaction phase}.}
%     \label{fig:interaction}
% \end{figure}
% %
% \begin{figure}[b]
%    \centering
%      \begin{subfigure}{0.2\columnwidth}
%      \centering
%     \includegraphics[height=2.5cm]{imagines/pdfs/joints.pdf}
%     \caption{}
%     \label{fig:joints}
% \end{subfigure}
% \begin{subfigure}{0.78\columnwidth}\centering
%    \includegraphics[height=3cm]{imagines/plots/joint_torque.pdf}
%     \caption{}
%     \label{fig:joint_torques}
% \end{subfigure}
% \caption{\new{(a) A simplified schematic of the 2-\ac{dof} manipulator. (b) \textbf{Task 2}: the 2-\ac{dof} manipulator joint torque magnitude $\tau_1$ and $\tau_2$ in two different scenarios: displaced \ac{com} and non-displaced \ac{com}.}}
% \label{fig:benchmark}
%     %\vspace{-0.5cm}
% \end{figure}
% \new{\subsection{\textbf{Task 1}}}
% \new{This section presents the testing results for a pushing task on a vertical surface using only the alignment frame, validating the feasibility of the proposed \ac{com} self-displacing approach.} A set of way-points \new{culminating with} points \enquote{behind} the work surface was sent to the high-level impedance controller to approach and \new{establish a }contact with the work surface using the alignment frame. Once stable contact between the system and the work surface was obtained, the \new{\ac{com} self-displacing process} was enabled. The shifting-mass \new{plate} position $l$ changed along the \new{positive} body axis $\bm{x}_B$ starting from its initial value $l=0$\si{\meter} while the back rotors tilting angle $\alpha$ was increasing, see \new{Fig.}~\ref{fig:interaction} Zone~1.

% In Zone~2, the \new{\ac{com} self-displacing} was completed with $\alpha\approx90\degree$\new{:} the shifting-mass \new{plate} reached a position at $l=0.25$\si{\meter} and kept increasing until the \new{ideal} position at $l^*=0.281$\si{\meter}. It maintained this position while exerting horizontal forces on the vertical surface using the full thrust of back rotors. Afterward, the shifting-mass \new{plate} returned to its initial position while the tilting angle $\alpha$ was decreasing, as in Zone~3. \new{The determined \new{ideal} shifting-mass \new{plate} position $l^*$ from the simulation can assist in setting the maximum allowed shifting-mass plate position in the physical experiments to prevent instability due to \ac{com} over-displacement.}

% The gain values $k_{\alpha}$ and $k_{\alpha I}$ are pivotal and need adjustment when there are changes in mass distribution. \new{In practice, having over-displaced \ac{com} (i.e. $d>L$) is highly risky. Therefore, smaller gain values are suggested at the beginning of the gain tuning process with the real platform to prevent damage. In the future, we will look into safely identifying the maximum \ac{com} displacement with the physical platform.} Moreover, from \new{Fig.}~\ref{fig:interaction}, a range of $l\in[0.25 \ 0.281]$\si{\meter} can enable $\alpha\approx90 \degree$ instead of a single value of $l^*$. Further analysis is warranted, taking into account friction forces between the alignment frame and the work surface.

% \new{\subsection{\textbf{Task 2}}}
% \new{In this task, the attached 2-\ac{dof} manipulator was used to push on the work surface under two scenarios: scenario (a) - displaced \ac{com}, and scenario (b) - non-displaced \ac{com}. In scenario (a), the shifting-mass plate equipped with the manipulator was shifted to its ideal position $l^*=0.28$\si{\meter} identified in \textbf{Task 1}. Operating close to the work surface with the maximum \ac{com} displacement allowed shorter beams of the manipulator. In this scenario, the manipulator was designed with $L_1=L_2=0.05$\si{\meter}. In scenario (b), the shifting-mass plate maintained its initial position, i.e. there was no \ac{com} displacement (the change of the system \ac{com} due to different arm configuration was not considered). In this case, longer beams were used for the manipulator with $L_1=L_2=0.2$\si{\meter} which are three times longer than the ones in scenario (a).}

% \new{In both scenarios, the manipulator was required to exert a $5$\si{\newton} pushing force normal to the work surface, for the manipulator control we refer to \cite{siciliano}. The joint torque magnitude of the manipulator for both scenarios is displayed in Fig.~\ref{fig:joint_torques}. In scenario (b), the joint torque magnitude reached $0.4$\si{\newton\meter} which is significantly larger than the magnitude in scenario (a), as expected in Sec.~\ref{sec:optimized_config}. With the simulation results, we validated the system design and control techniques promising the following physical implementation. The simulation illustrating the desired operational flow as in Fig.~\ref{fig:aero_bull} is shown in Part 1 of the accompanying video\footnote{\url{https://youtu.be/M25WdeowUNk}}.}

